${\rm S{\scriptsize IM}BIG}$: The First Cosmological Constraints from the Non-Linear Galaxy Bispectrum

We present the first cosmological constraints from analyzing higher-order galaxy clustering on non-linear scales. We use ${\rm S{\scriptsize IM}BIG}$, a forward modeling framework for galaxy clustering analyses that employs simulation-based inference to perform highly efficient cosmological inference using normalizing flows. It leverages the predictive power of high-fidelity simulations and robustly extracts cosmological information from regimes inaccessible with current standard analyses. In this work, we apply ${\rm S{\scriptsize IM}BIG}$ to a subset of the BOSS galaxy sample and analyze the redshift-space bispectrum monopole, $B_0(k_1, k_2, k_3)$, to $k_{\rm max}=0.5\,h/{\rm Mpc}$. We achieve 1$\sigma$ constraints of $\Omega_m=0.293^{+0.027}_{-0.027}$ and $\sigma_8= 0.783^{+0.040}_{-0.038}$, which are more than 1.2 and 2.4$\times$ tighter than constraints from standard power spectrum analyses of the same dataset. We also derive 1.4, 1.4, 1.7$\times$ tighter constraints on $\Omega_b$, $h$, $n_s$. This improvement comes from additional cosmological information in higher-order clustering on non-linear scales and, for $\sigma_8$, is equivalent to the gain expected from a standard analysis on a $\sim$4$\times$ larger galaxy sample. Even with our BOSS subsample, which only spans 10% of the full BOSS volume, we derive competitive constraints on the growth of structure: $S_8 = 0.774^{+0.056}_{-0.053}$. Our constraint is consistent with results from both cosmic microwave background and weak lensing. Combined with a $\omega_b$ prior from Big Bang Nucleosynthesis, we also derive a constraint on $H_0=67.6^{+2.2}_{-1.8}\,{\rm km\,s^{-1}\,Mpc^{-1}}$ that is consistent with early universe constraints.

==> valid.tex <==
\section{Posterior Validation}  \label{sec:cross}
In this appendix, we demonstrate that our \simbig~$B_0$ posterior estimate, 
$q_{\bphi}$ is sufficiently accurate for the $\Lambda$CDM cosmological paramters. 
We also demonstrate that the \simbig~forward model provides enough flexibility
to infer unbiased cosmological constraints using the $B_0(k_{123})$.
We make use of 2,000 test simulations in the three test sets described in 
\cite{simbig_mock}: $\mathtt{TEST0}, \mathtt{TEST1}$,  and  $\mathtt{TEST2}$.
Each test set is constructed using a different forward model. 
The 500 $\mathtt{TEST0}$ simulations use the same forward model as the training set: 
{\sc Quijote} $N$-body, {\sc Rockstar} halo finder, and the full \simbig~HOD. 
The 500 $\mathtt{TEST1}$ simulations use {\sc Quijote} $N$-body, Friend-of-Friend halo 
finder, and the simpler \cite{zheng2007} HOD model. 
Lastly, the 1,000 $\mathtt{TEST2}$ simulations use {\sc AbacusSummit} $N$-body 
simulations~\citep{maksimova2021}, {\sc CompaSO} halo finder~\citep{hadzhiyska2022}, 
and the full \simbig~HOD.

\simbig~uses SBI based on neural density estimation to estimate the 
posterior of cosmological parameters for given a summary statistic 
of the observed galaxy distribution. 
Neural density estimation minimizes the KL divergence between the 
posterior estimate and the true posterior. 
So in the ideal limit of an infinitely large training set and with 
successful minimization, the neural posterior estimate would perfectly 
estimate the true posterior. 
Unfortunately, in our case we have a limited training set of 20,000 
forward modeled simulations. 
Hence, we further validate the accuracy of our posterior estimate. 

\begin{figure}
\begin{center}
    \includegraphics[width=\textwidth]{test_posteriors.pdf}
    \caption{\label{fig:test_post}
    Posteriors of $(\Omega_m, \sigma_8)$ inferred using the \simbig~bispectrum 
    analysis for a random subset of the $\mathtt{TEST0}$ (top), $\mathtt{TEST1}$ 
    (center), and  $\mathtt{TEST2}$ (bottom) simulations.
    We mark the 68 and 84 percentiles of the posteriors with the contours. 
    We also include the true $(\Omega_m, \sigma_8)$ of the test simulations in
    each panel (black $\times$). 
    The comparison between the posteriors and the true parameter values
    qualitatively show good agreement for each test simulation. 
    }
\end{center}
\end{figure}

We run the \simbig~posterior estimate on all of the test simulations
and derive a posterior for each simulation. 
In Figure~\ref{fig:test_post}, we present the $(\Omega_m, \sigma_8)$ 
posteriors for a randomly selected subset of the test  simulations. 
We present posteriors for $\mathtt{TEST0}$, $\mathtt{TEST1}$, and
$\mathtt{TEST2}$ simulations in the top, center, and bottom panels. 
The contours represent the 68 and 95 percentiles of the posteriors. 
In each panel, we mark the true $(\Omega_m, \sigma_8)$ value of the test
simulation (black x). 
Each test simulation is a unique realization of a CMASS-like galaxy catalog
subject to cosmic and statistical variance. 
We, therefore, do not expect the true $(\Omega_m, \sigma_8)$ value to lie at
the center of each of the posteriors. 
Instead, we note that for the majority of the randomly selected test
simulations, the true parameter values lie within the 68 and 95 percentiles
\simbig~posteriors. 

\begin{figure}
\begin{center}
    \includegraphics[width=\textwidth]{sbc.pdf}
    \caption{\label{fig:sbc}
        SBC validation of the \simbig~$B_0(k_{123} < 0.5\,h/{\rm Mpc})$ posterior 
        estimate. 
        We present the distribution of the rank statistics, which are derived 
        by comparing the true parameter values to the inferred marginalized 1D
        posteriors. 
        The rank statistics are calculated using 2,000 validation simulations 
        that were excluded from training the posterior estimate. 
        For an accurate estimate of the true posterior, the rank statistic would 
        be uniformly distributed (black dashed). 
        Overall, we accurately estimate the posterior of all of the $\Lambda$CDM 
        cosmological parameters. 
    }
\end{center}
\end{figure}

Next, we assess the accuracy and precision of the \simbig~more quantitatively.
In \cite{simbig_mock}, they used simulation-based calibration~\citep[SBC;][]{talts2020} 
with rank statistics, or coverage, to assess the accuracy and robustness of 
the posterior estimates. 
This assessment, however, requires that the parameters of the test simulations 
sample the full prior distribution. 
Otherwise, the distribution of the rank statistic is {\em not} guaranteed to be 
uniform, even for the true posterior. 
The test simulations are evaluated at fiducial values of the cosmological 
parameters.
$\mathtt{TEST0}$ and $\mathtt{TEST1}$ are run at: 
$\Omega_m = 0.3175, \Omega_b = 0.049, h = 0.6711, n_s = 0.9624, \sigma_8 = 0.834$.
$\mathtt{TEST2}$ are run at: 
$\Omega_m = 0.3152, \Omega_b = 0.049, h = 0.6736, n_s = 0.9649, \sigma_8 = 0.808$.

We, instead, use the 2,000 validation simulations that were excluded from the
training of our posterior estimate (Section~\ref{sec:sbi}). 
In Figure~\ref{fig:sbc}, we present the SBC rank statistic distribution for
the $\Lambda$CDM cosmological parameters. 
For each simulation and cosmological parameter, we calculate the rank of the 
true parameter value within the marginalized 1D posterior estimate. 
Since the validation simulations span the full prior, a uniform rank statistic 
distribution indicates that we accurately estimate the true posterior (black dashed).
Overall, the rank distributions are close to uniform for all of the $\Lambda$CDM 
cosmological parameters. 
For $\Omega_m$ and $\sigma_8$, the distribution have a slight $\cap$-shape. 
This suggests that our $\Omega_m$ and $\sigma_8$ posterior estimates are slightly 
broader than the true posterior. 
We, therefore, conclude that our \simbig~$B_0$ posterior is sufficiently accurate.

\begin{figure}
\begin{center}
    \includegraphics[width=\textwidth]{valid_posterior_mean.pdf}
    \caption{\label{fig:postmean}
    Comparison of the compressed bispectrum likelihood, 
    $p(B_0^{(c)}\given \theta_{\rm fid})$,  computed on the three sets of 
    test simulations: 
    $\mathtt{TEST0}$ (blue), $\mathtt{TEST1}$ (orange), and
    $\mathtt{TEST2}$ (green).
    $B_0^{(c)}$ is derived by taking the mean of the marginalized 1D 
    \simbig~$B_0$ posterior for the $\Lambda$CDM parameters, an optimal
    compression of the cosmological information in $B_0$. 
    In each panel, we mark the corresponding $\Lambda$CDM parameters.
    The likelihoods are at the fixed fiducial cosmologies and parameter
    values of the test sets. 
    We present the distribution of $B_0^{(c)} - \overline{B_0^{(c)}}$
    because $\mathtt{TEST2}$ simulations are constructed using different 
    fiducial parameter values than the $\mathtt{TEST0}$ and
    $\mathtt{TEST1}$ simulations.
    Overall, {\em we find excellent agreement among the likelihoods
    of the different test simulations and conclude that our $B_0$ 
    analysis is robust to modeling choices in our forward model}.
    }
\end{center}
\end{figure}

In addition to validating the accuracy of our posterior estimate, we also
assess the robustness of our $B_0$ analysis. 
The \simbig~forward model for the galaxy distribution, or {\em any} forward model, 
makes modeling choices and assumptions that, in detail, do not reflect the 
actual Universe. 
To account for this limitation, \simbig~is designed to be highly flexible so
that we can robustly marginalize over the complex physical processes that govern
galaxy formation and the galaxy-halo connection.  
Nevertheless, a summary statistic of the galaxy distribution may be sensitive to 
the specific choices made in the forward model.
More importantly, this can bias the inferred cosmological parameters. 
We therefore assess whether $B_0$ is sensitive to the forward model and validate 
that we can derive unbiased cosmological parameter constraints. 

To assess the robustness of $B_0$, we want to compare the likelihoods predicted
by the different test sets. 
If $B_0$ is sensitive to variations in the forward model, there will be significant
discrepancies among the likelihoods predicted by different forward models. 
With our test suite, we can check for these discrepancies in three different 
forward models. 
In practice, however, comparing the $B_0$ likelihood presents significant 
challenges.
The likelihood is a distribution over the summary statistics space and, thus, 
has the same dimensionality as the 10,052-dimensional
$B_0(k_{123} < 0.5\,h/{\rm Mpc})$.

Instead, we compare the likelihoods of the compressed $B_0$, $B_0^{(c)}$, for 
$\mathtt{TEST0}$ (blue), $\mathtt{TEST1}$ (orange), and $\mathtt{TEST2}$ (green) 
in Figure~\ref{fig:postmean}.
For the compression, we use the mean of the marginalized 1D \simbig~$B_0$ posterior 
for the $\Lambda$CDM cosmological parameters: 
$B_0^{(c)} = \sum_{j=1}^{N} \btheta_j/N$ where $\btheta_j \sim q_{\bphi}(\btheta\given B_0)$.
Each panel represents the mean corresponding to one of the $\Lambda$CDM parameters.
This is an optimal compression of the  cosmological information in $B_0$, since 
$q_{\bphi}$ accurately estimates the true posterior, as we demonstrate above.
Since, the $\mathtt{TEST2}$ simulations are constructed using a different set of 
fiducial parameter values than the $\mathtt{TEST0}$ and $\mathtt{TEST1}$ simulations,
we present the distribution of $B_0^{(c)} - \overline{B_0^{(c)}}$, where 
$\overline{B_0^{(c)}}$ is the average $B_0^{(c)}$.
Overall, we find excellent agreement among the $B_0^{(c)}$ likelihoods with no
significant discrepancies.
We also find similar levels of agreement when we use other summaries of the 
marginalized \simbig~$B_0$ posterior (\emph{e.g.} standard deviation, 16$^{\rm th}$ percentile)
for the compression. 
Given the good agreement of $B_0^{(c)}$ likelihoods among the test sets,
we conclude that our $B_0$ analysis is sufficiently robust to the modeling choices 
in our forward model.

% discuss ways the validation could be better. 
We note that our likelihood comparison only demonstrates robustness near the 
fiducial cosmologies of the test simulations. 
Furthermore, some cosmological information may be lost in the $q_{\bphi}$-based 
compression scheme, which may underestimate the discrepancies in the full $B_0$ 
likelihood.
Addressing either of these limitations, however, will require a substantially 
larger suite of simulations evaluated across the full prior space. 
We reserve developing more stringent and efficient validation of the posterior and 
summary statistic to future work. 

